APPLS: Evaluating Evaluation Metrics for Plain Language Summarization

While there has been significant development of models for Plain Language Summarization (PLS), evaluation remains a challenge. PLS lacks a dedicated assessment metric, and the suitability of text generation evaluation metrics is unclear due to the unique transformations involved (e.g., adding background explanations, removing jargon). To address these questions, our study introduces a granular meta-evaluation testbed, APPLS, designed to evaluate metrics for PLS. We identify four PLS criteria from previous work -- informativeness, simplification, coherence, and faithfulness -- and define a set of perturbations corresponding to these criteria that sensitive metrics should be able to detect. We apply these perturbations to extractive hypotheses for two PLS datasets to form our testbed. Using APPLS, we assess performance of 14 metrics, including automated scores, lexical features, and LLM prompt-based evaluations. Our analysis reveals that while some current metrics show sensitivity to specific criteria, no single method captures all four criteria simultaneously. We therefore recommend a suite of automated metrics be used to capture PLS quality along all relevant criteria. This work contributes the first meta-evaluation testbed for PLS and a comprehensive evaluation of existing metrics. APPLS and our evaluation code is available at https://github.com/LinguisticAnomalies/APPLS.

==> old/acl_reported_results.tex <==
\section{Empirical Study of Evaluation Metrics Reported in ACL 2022 Publications}

% \begin{figure*}[h!]
%     \centering
%     \includegraphics[trim={1cm 10cm 5cm 8cm}, clip, scale=0.25]{emnlp2023-latex/figures/acl_whole.pdf}
%     \caption{Results from an empirical study of ACL 2022 papers: a. frequency of metrics reported for summarization and generation tasks; b. reported metric improvements for the proposed model relative to the baseline; and c. ratio of median improvement to the score variation at 100\% perturbation. Green shades represent a opposite direction to the score change induced by perturbation, while orange shades signify the same direction.}
%     \label{fig:acl_whole}
% \end{figure*}

Our study undertakes a comprehensive analysis of scores reported in the long papers of ACL 2022 to identify the most prevalently utilized metrics in summarization and simplification tasks. We primarily concentrate on tasks related to generation, summarization, and simplification. Our inclusion criteria are: 1) long papers with 'generat,' 'summar,' or 'simpl' in the title; 2) papers that report scores for both the current model and at least one baseline model in the main text. We exclude scores from ablation studies. 
\begin{figure}[h]
    \centering
    \includegraphics{emnlp2023-latex/figures/reported_score_count.pdf}
    \caption{Caption}
    \label{fig:reported_score_count}
\end{figure}

Of the 601 long papers, 109 conform to our inclusion criteria, categorized into 31 summarization and 78 generation tasks, with no qualified papers related to simplification tasks. Considering the significance of simplification in PLS, we expanded our search to all ACL 2022 papers, including long, short, sustem demonstration, and findings. This led to the identification of 2 out of 22 papers with 'simpl' in the title that reported SARI scores. As illustrated in Figure \ref{fig:reported_score_count}, the five most frequently reported automated evaluation metrics are ROUGE, BLEU, GPT-PPL, METEOR, and BERTScore.

\begin{figure}[h]
    \centering
    \includegraphics[]{emnlp2023-latex/figures/acl_score_improvement.pdf}
    \caption{Caption}
    \label{fig:acl_score_improvement}
\end{figure}
Our analysis also extends to how the reported scores vary between the baseline and proposed models. The median reported improvements for the identified metrics and SARI in qualified papers are 0.89, 0.69, 2.06, 0.50, 0.55, and 1.71, respectively, as shown in \ref{fig:acl_score_improvement}. 

This investigation provides an insightful perspective on the current adoption of evaluation metrics in natural language generation, summarization, and simplification tasks. We observe that a majority of papers employ the same metrics across these tasks, and the reported improvements are often minor compared to the originally proposed range (0-100) for each measure. Given the typical treatment of the PLS task as a summarization or simplification task, these findings underscore the necessity for a more discerning choice of metrics, highlighting the importance of comprehending the significance and implications of score differences in these widely adopted evaluation metrics.

% The subsequent question is whether these differences imply significant changes in the text. We compare the reported improvements to the full perturbation of the text and analyze their implications. Results are discussed in Section \ref{score_change_acl_20222}.


==> old/conclusion.tex <==
\section{Conclusion}

Recent advances in NLP point to the possibility of automated plain language summarization (PLS); however, the multifaceted nature of PLS has complicated efforts to define useful evaluation criteria. We present a novel granular testbed, \testbed, for evaluating evaluation metrics in the context of PLS. Using \testbed, we show that most existing metrics struggle to effectively capture a major criteria of PLS: simplification. We address this gap with \plainscore, a novel evaluation metric using normalized LM perplexity differences to assess simplification. \plainscore accurately captures simplification perturbations in our testbed and demonstrates strong performance on several simplification datasets. It is our hope that the methods and metrics development introduced in this work could be generalized beyond medical PLS to facilitate better evaluation for other text generation tasks. Our testbed and metric also lay the groundwork for further advancements in automated PLS, with the hope of facilitating more impactful, accessible, and equitable scientific communication. 

% Plain language summarization (PLS) of scientific information is necessary to


% \plainscore uses the normalized difference between in-domain and out-of-domain language model perplexities, allowing the metric to effectively measure simplification without the limitations of a previous perplexity-based metrics (e.g., sensitivity to text length). 


% \testbed applies incremental perturbations to a dataset, where each type of perturbation is associated with a criteria that an evaluation metric for PLS should be sensitive to.



% Future research should continue to explore and refine evaluation metrics, taking into account the specific criteria of various text generation tasks. As the field of natural language processing continues to evolve, it is vital that evaluation methodologies keep pace to ensure the accurate and meaningful assessment of generated text.

% By employing our proposed pipeline, we can better understand the strengths and limitations of evaluation metrics and algorithms across various text generation tasks. 



==> old/create_perturbations_old.tex <==
\section{Criteria-specific Perturbation Design}
\label{criteria_specific_perturbation_design}

To assess existing metric sensitivity to our proposed criteria, we develop the following perturbations (illustrative examples in Table~\ref{table:perturbation_example}). We define sensitivity similar to prior work \citep{gabriel2020go} as being correlated in the correct direction with the amount of perturbation. 

\subsection{Informativeness}

\paragraph{Delete sentences} We simulate the omission of crucial information by ranking sentences based on similarity to others (assuming more similar is more likely to contain important information) \citep{zhong2020discourse} and removing sentences starting from the most to least similar. 

\vspace{-2mm}
\paragraph{Add sentences} We simulate the inclusion of two forms of unrelated information by adding sentences from \textit{out-of-domain} (i.e., unrelated dataset) and \textit{in-domain} (i.e., within the same domain but on a different topic).

\vspace{-2mm}
\paragraph{Add definitions} Background explanation is fundamental to PLS and involves adding external content such as definitions or examples \citep{guo2022cells, srikanth2020elaborative}. To simulate this phenomenon, we add definitions\footnote{Taken from \href{http://wikidata.dbpedia.org/develop/datasets}{http://wikidata.dbpedia.org/develop/datasets}} of keywords identified by KeyBERT \citep{grootendorst2020keybert}.

\subsection{Simplification}
\paragraph{Replace sentences} Taking advantage of the GPT-series models' ability to simplify text \citep{Lu2023NapSSPM}, we replace sentences in the original text with GPT-simplified versions. We use the \textit{text-davinci-003} model to generate simplified summaries using the prompt {\texttt{``explain the text in layman's terms to a primary school student.''}} GPT configurations can be found in App.~\ref{sec:gpt_generation_setup}. 

\subsection{Coherence}
\paragraph{Reorder sentences} We simulate changes in text coherence by randomly shuffling the order of sentences, as suggested by \citet{sai2021perturbation}. 

\subsection{Faithfulness}

\paragraph{Number swap} We randomly add a number from 1 to 5 to the original numerical value in the text.

\vspace{-2mm}
\paragraph{Verb swap} An appropriate metric should exhibit constancy for synonymous verbs but sensitivity for antonymous ones. Hence, we introduce two perturbations, where identify verbs and substitute them with either synonyms or antonyms.

\vspace{-2mm}
\paragraph{Entity swap} We replace entities using the KBIN method \cite{wright2022generating}, which links entity spans to concepts in the Unified Medical Language System (UMLS) and replaces them with different entities while maximizing NLI contradiction and minimizing LM perplexity. This results in a fluent sentence that contradicts the original one.

\vspace{-2mm}
\paragraph{Negate sentences} We negate sentences by identifying verbs and adding negation terms (e.g., not) preceding them. The goal of this perturbation is to create sentences similar to the original but communicating the exact opposite information. 



==> old/desired_criteria.tex <==
\section{Desired Criteria for PLS Metric} \label{desired_criteria_and_perturbations}

\begin{table*}
  \includegraphics[trim={12cm 3cm 12cm 3cm},clip, scale=0.36]{emnlp2023-latex/figures/perturbation_example.pdf}
  \vspace{-2mm}
  \caption{Example perturbations for criteria in APPLS. Original text comes from the CELLS \cite{guo2022cells}. The hypothetical criteria change direction with perturbation is denoted as arrows. }
  \label{table:perturbation_example}
\end{table*}

We define four criteria that an effective evaluation metric for PLS should be sensitive to in Table~\ref{desire_criteria}. These criteria are informed by both abstractive summarization \citep{sai2022survey} and plain language summarization paradigms \cite{pitcher2022template, ondov2022survey, stoll2022plain, jain2022survey}. \\[-4mm]

% \noindent \textbf{Informativeness} measures the extent to which a plain language summary covers essential information such as methodology, primary findings, and conclusions in the original text. An informative summary conveys the central messages of the text, and does not remove crucial details \citep{Devaraj2022EvaluatingFI, pitcher2022template} or hallucinate \citep{Maynez2020OnFA, Goyal2021AnnotatingAM}. \textit{We hypothesize that an ideal metric should decrease with the elimination of notable sentences and the insertion of irrelevant sentences, and increase with the incorporation of relevant definitions.} \\[-4mm]

% \noindent \textbf{Simplification} describes the degree to which information is conveyed in a form that non-expert audiences can readily understand. This criterion prioritizes the use of simple vocabulary \citep{bingel2018lexi, laban2021keep}, casual language \citep{pitcher2022template}, and concise sentences \citep{de2010text, scarton2018text} that minimize excessive jargon and technical terminology unfamiliar to a lay audience.\footnote{Text simplification is its own distinct task; in comparison to the PLS task, text simplification focuses on surface-level changes to simplify language and does not involve other relevant criteria important to PLS (e.g., informativeness).} Reducing complexity by substituting complex sentences with simpler ones has been empirically shown to reduce the difficulty of text \citep{van2019evaluating}. \textit{We hypothesize that an ideal metric should exhibit sensitivity towards the substitution of complex sentences with simplified counterparts in the text.} \\[-4mm]

% \noindent \textbf{Coherence} describes the logical arrangement of a plain language summary. A coherent summary presents information in a well-ordered fashion that facilitates ease of comprehension for the reader \citep{mcnamara2001, sai2022survey}. \citet{barzilay2002inferring} underscored the significance of sentence sequencing in affecting user comprehension. We conjecture that the original sentence order reflects optimal coherence. \textit{Consequently, we hypothesize that an ideal metric should demonstrate sensitivity to modifications in sentence sequencing.} \\[-4mm]

% \noindent \textbf{Faithfulness} denotes how well the plain language summary aligns factually with the source text. A faithful summary should not substitute information or introduce errors, misconceptions, and inaccuracies \citep{Devaraj2022EvaluatingFI, Prabhakaran2019PerturbationSA}. Faithfulness focuses on factual alignment, while informativeness measures the completeness and efficiency of the summary in conveying key points. 
% \textit{We hypothesize that an ideal metric should exhibit sensitivity towards changes in factual information such as entity swaps and sentence negation, while maintaining indifference to synonym swaps.}







==> old/existing_metrics_old.tex <==
% \input{emnlp2023-latex/tables/lexical_feature_slope}

% \begin{table*}
%   \includegraphics[trim={15cm 10cm 15cm 7cm},clip, scale=0.4]{emnlp2023-latex/figures/automated_metrics_slope.pdf}
%   \caption{Example text subject to perturbations.}
%   \label{table:automated_metrics_slope}
% \end{table*}

% \begin{table*}
%   \includegraphics[trim={15cm 10cm 13cm 7cm},clip, scale=0.4]{emnlp2023-latex/figures/automated_metrics_slope_underline.pdf}
%   \caption{Example text subject to perturbations.}
%   \label{table:automated_metrics_slope}
% \end{table*}



\section{Existing Metrics We Evaluate}
\label{existing_metrics}
Our analysis spans eight established evaluation metrics, including five metrics most commonly reported in ACL'22 summarization and generation papers (empirical results in App.~\ref{acl_appendix}) and three additional metrics
(\S\ref{sec:existing_automated_evaluation_metrics}). We also assess five lexical features associated with text simplification (\S\ref{sec:lexical_feature_baed_metrics}) and LLM-based evaluations (\S\ref{sec:promptbased}). 


\subsection{Existing automated evaluation metrics}
\label{sec:existing_automated_evaluation_metrics}

\noindent \textbf{Overlap-based metrics} measure $n$-gram overlaps, and are popular due to their ease of use.
\begin{itemize}[noitemsep, topsep=1pt, leftmargin=10pt]
\item \textbf{ROUGE}\footnote{Implementation: \citet{fabbri2021summeval}\label{summeval}} \cite{lin2004rouge} measures $n$-gram overlap between generated and reference summaries, focusing on recall. We report the average of ROUGE-1, ROUGE-2, and ROUGE-L.
\item \textbf{BLEU}\footref{summeval} \cite{papineni2002bleu} computes $n$-gram precision of generated text against reference texts, including a brevity penalty.
\item \textbf{METEOR}\footref{summeval} \cite{banerjee2005meteor} employs a relaxed matching criterion based on the F-measure, and addresses the exact match restrictions and recall consideration of BLEU.
\item \textbf{SARI}\footnote{Implementation: \citet{alva-manchego-etal-2019-easse}\label{easse}} \cite{xu2016optimizing}  is specifically designed to evaluate text simplification tasks. The score weights deleted, added, and kept $n$-grams between the source and target texts.
\end{itemize}

\noindent \textbf{Model-based metrics} use pretrained models to evaluate text quality.
\begin{itemize}[noitemsep, topsep=1pt, leftmargin=10pt]
\item \textbf{GPT-PPL},\footnote{\href{https://huggingface.co/transformers/v3.2.0/perplexity.html}{https://huggingface.co/transformers/v3.2.0/perplexity.html}} usually computed with GPT-2, measures fluency and coherence by calculating the average log probability assigned to each token by the GPT model, with lower scores indicating higher fluency and coherence.
\item \textbf{BERTScore}\footref{summeval} \cite{zhang2019bertscore} quantifies the similarity between hypothesis and targets using contextualized embeddings from the BERT model, computing the F1-score between embeddings to capture semantic similarity beyond $n$-gram matching.
\item \textbf{LENS} \cite{maddela2022lens} employs an adaptive ranking loss to focus on targets closer to the system output in edit operations (e.g., splitting, paraphrasing, deletion).
\end{itemize}

\noindent \textbf{QA-based metrics} capture content quality using a question-answering approach. 
\begin{itemize}[noitemsep, topsep=1pt, leftmargin=10pt]
\item \textbf{QAEval} \cite{deutsch2021towards} generates question-answer pairs from the target text, then uses a learned QA model to answer these questions using the generated text. The score is computed as the proportion of questions answered correctly. We report QAEval LERC scores.
\end{itemize}

\subsection{Lexical features} 
\label{sec:lexical_feature_baed_metrics}
We also assess lexical features that have been shown to be predictive of text simplicity:
\begin{itemize}[noitemsep, topsep=1pt, leftmargin=10pt]
\item \textbf{Length}: Shorter sentences are easier to understand \cite{kauchak2017measuring}. We report both sentence length and paragraph length.
\item \textbf{Familiarity}: Simple text contains more common words \cite{leroy2018next}. We compute the percentage of text that is made up of the 1,000 most common English words.\footnote{\href{https://gist.github.com/deekayen/4148741}{https://gist.github.com/deekayen/4148741}}
\item \textbf{Specificity}: For biomedical text, MeSH term depth is predictive of sentence difficulty \cite{kauchak2014text}. MeSH terms are used to index articles in PubMed, and we determine the depth of an article's terms by splitting term identifiers on `.' (e.g., term depth for Zika Virus with identifier B04.820.578.344.350.995 is 6). 
\item \textbf{Phrase Transitions}: Conjunctions (e.g., therefore) are important for flow and can assist with comprehension \cite{kauchak2017measuring}. We report the number of conjunctions.
\item \textbf{Function Words}: Simple text contains more verbs and fewer nouns \cite{mukherjee2017role}. We report the number of verbs, nouns, adjectives, adverbs, and numbers.

\end{itemize}

\subsection{LLM prompt-based evaluations}
\label{sec:promptbased}
Prompting LLMs for text generation evaluation has been explored in recent work \cite{gao2023human, luo2023chatgpt}. We adopt the template from \citet{gao2023human}, prompting GPT-3 (\textit{text-davinci-003}) to evaluate the hypotheses in our testbed across four dimensions---informativeness, simplification, coherence, and faithfulness---and provide an overall quality score. All scores are from 0 (worst) to 100 (best). We supply the definitions for each criterion in the prompt. 

We test two experimental settings: one in which we only provide the source abstract (reference-free), and the other in which both the source abstract and the target plain language summary are provided (reference-provided). Model configurations and prompt details are available in App.~\ref{sec:prompt_based_evaluation_appendix}.

==> tables/cells_dataset_description.tex <==
\begin{table}
\small
\centering
\begin{tabular}{@{}l l l l l @{}}
\toprule
 & \textbf{Src.} & \textbf{Tgt.} & \textbf{Oracle} & \textbf{GPT}\\
\midrule
\textbf{Avg. \# words}  & 283 & 178 & 134 & 98\\
\textbf{Avg. \# sentences} & 11 & 7  & 5 & 4\\
\textbf{Vocabulary size} & 76,275 & 46,522 &  46,658 & 27,937\\
\bottomrule
\end{tabular}
\caption{CELLS test set (n=6,311) statistics for source (abstract), target (plain language summary), oracle extractive hypothesis, and GPT-simplified summaries.}
\label{cells_dataset}
\end{table}

==> tables/desired_criteria.tex <==
\begin{table}
\small
\begin{tabular}{@{}m{2cm}m{5cm}@{}}
\toprule
\textbf{Criterion}  & \textbf{Description} \\
\midrule
\textbf{Informativeness} & The extent to which a plain language summary covers essential information such as methodology, primary findings, and conclusions in the original text.\\
\midrule
\textbf{Simplification}  & The degree to which information is conveyed in a form that non-expert audiences can readily understand.\footnote{Text simplification is its own distinct task; in comparison to the PLS task, text simplification focuses on surface-level changes to simplify language and does not involve other relevant criteria important to PLS (e.g., informativeness).}\\
\midrule
\textbf{Coherence}   & The logical arrangement of a plain language summary.\\
\midrule
\textbf{Faithfulness}   & How well the plain language summary aligns factually with the source text. \\
\bottomrule
\end{tabular}
\caption{Desired criteria and its definition.}
\label{desire_criteria}
\end{table}


% \noindent \textbf{Informativeness} measures the extent to which a plain language summary covers essential information such as methodology, primary findings, and conclusions in the original text. An informative summary conveys the central messages of the text, and does not remove crucial details \citep{Devaraj2022EvaluatingFI, pitcher2022template} or hallucinate \citep{Maynez2020OnFA, Goyal2021AnnotatingAM}. \textit{We hypothesize that an ideal metric should decrease with the elimination of notable sentences and the insertion of irrelevant sentences, and increase with the incorporation of relevant definitions.} \\[-4mm]

% \noindent \textbf{Simplification} describes the degree to which information is conveyed in a form that non-expert audiences can readily understand. This criterion prioritizes the use of simple vocabulary \citep{bingel2018lexi, laban2021keep}, casual language \citep{pitcher2022template}, and concise sentences \citep{de2010text, scarton2018text} that minimize excessive jargon and technical terminology unfamiliar to a lay audience.\footnote{Text simplification is its own distinct task; in comparison to the PLS task, text simplification focuses on surface-level changes to simplify language and does not involve other relevant criteria important to PLS (e.g., informativeness).} Reducing complexity by substituting complex sentences with simpler ones has been empirically shown to reduce the difficulty of text \citep{van2019evaluating}. \textit{We hypothesize that an ideal metric should exhibit sensitivity towards the substitution of complex sentences with simplified counterparts in the text.} \\[-4mm]

% \noindent \textbf{Coherence} describes the logical arrangement of a plain language summary. A coherent summary presents information in a well-ordered fashion that facilitates ease of comprehension for the reader \citep{mcnamara2001, sai2022survey}. \citet{barzilay2002inferring} underscored the significance of sentence sequencing in affecting user comprehension. We conjecture that the original sentence order reflects optimal coherence. \textit{Consequently, we hypothesize that an ideal metric should demonstrate sensitivity to modifications in sentence sequencing.} \\[-4mm]

% \noindent \textbf{Faithfulness} denotes how well the plain language summary aligns factually with the source text. A faithful summary should not substitute information or introduce errors, misconceptions, and inaccuracies \citep{Devaraj2022EvaluatingFI, Prabhakaran2019PerturbationSA}. Faithfulness focuses on factual alignment, while informativeness measures the completeness and efficiency of the summary in conveying key points. 
% \textit{We hypothesize that an ideal metric should exhibit sensitivity towards changes in factual information such as entity swaps and sentence negation, while maintaining indifference to synonym swaps.}

==> tables/gpt_overall_score.tex <==
\begin{table}[t!]
\centering
\small
\begin{tabular}{@{}lcc@{}}
\toprule
\multicolumn{1}{l}{}   & \textbf{Ref. Free}       & \textbf{Ref. Provided}    \\
\midrule
\textbf{Informativeness ($\downarrow$)}        &  &  \\
Delete sentence        & \textbf{-61.09}               & \textbf{-22.33}               \\
Add out-of-domain sent & \textbf{-19.91}               & \textbf{-34.88}               \\
Add in-domain sent     & \textbf{-7.32}                & -6.99                \\
Add definition ($\uparrow$) & -0.6 & 12.64 \\
\midrule
\textbf{Simplification ($\uparrow$)}         & -15.98              & -11.46              \\
\midrule
\textbf{Coherence ($\downarrow$)}              & -0.17                & -1.06                \\
\midrule
\textbf{Faithfulness ($\downarrow$)}           &  &  \\
Number swaps           & 0.45                 & -0.44                \\
Entity swaps           & \textbf{-5.48}                & -7.24                \\
Synonyms verb swaps    & -4.02                & -10.54              \\
Antonyms verb swaps    & \textbf{-6.05}                & \textbf{-8.27}                \\
Negate sentence        & \textbf{-18.59}               & \textbf{-21.94}              \\
\bottomrule
\end{tabular}
\caption{Overall score derived from the prompt-based evaluation for two settings: reference-free and reference-provided. \textbf{Bolded} values indicate statistical significance in the correct direction with Bonferroni-Holm correction for multiple hypothesis testing \cite{holm1979simple}.}
\label{gpt_overall_score}
\end{table}

==> tables/lexical_feature_slope.tex <==
\begin{table*}[h!]
% \scriptsize
\small
\centering
\begin{tabular}{@{} r rr r r r rrrrr}
\toprule
& \multicolumn{2}{c}{\bf{Length}} & \multicolumn{1}{c}{\bf{Familiarity}} & \multicolumn{1}{c}{\bf{Specificity}} & \bf{Trans.} & \multicolumn{5}{c}{\bf{Function Words}} \\
\cmidrule(lr){2-3}
\cmidrule(lr){4-4}
\cmidrule(lr){5-5}
\cmidrule(lr){6-6} 
\cmidrule(lr){7-11}
& Para. & Sent. & Common Words & MeSH Terms & Conj. & V. & N. & Adj. & Adv. & Num.  \\
\midrule

\textbf{Simplification} & -41.63 & -5.22 & 0.12 & -0.90 & -0.01 & 0.06 & -0.05 & -0.04 & 0 & 0 \\

\bottomrule
\end{tabular}

\caption{Slope coefficients of linear regression between perturbation percentage and lexical feature-based metrics for CELLS. The slopes represent the estimated change in evaluation score for a 100\% perturbation.  All  values are statistically significant with Bonferroni-Holm correction for multiple hypothesis testing \cite{holm1979simple}.}
\label{lexical_feature_slope}
\end{table*}

==> tables/perturbation_slope.tex <==
\begin{table*}[h!]
\small
\centering
\begin{tabular}{@{} m{3cm} rrrr rrr r r @{}}
\toprule
& \multicolumn{4}{c}{\bf{Overlap-based}} & \multicolumn{3}{c}{\bf{Model-based}} & \bf{QA-based} & \multicolumn{1}{c}{\bf{New}} \\
\cmidrule(lr){2-5}
\cmidrule(lr){6-8}
\cmidrule(lr){9-9}
\cmidrule(lr){10-10} 
\multicolumn{1}{c}{}
& ROUGE & BLEU & METEOR & SARI & BERTSc. & PPL($\downarrow$) & LENS & QAEval & \plainscore \\
\midrule
\textbf{Informativeness ($\downarrow$)} & & & & & & & \\
Delete sentence & \textbf{-25.19} & \textbf{-11.16}  & \textbf{-0.18} & \textbf{-5.24} & \textbf{-16.78} & \textbf{82.79} & 1.41 & \textbf{-0.95} & 5.89 \\
Add out-of-domain sent & \textbf{-5.23} & \textbf{-2.07} & 0.01 & -0.06  & \textbf{-5.26} & \textbf{49.41}  & 0 & \textbf{-0.19} & -0.1 \\
Add in-domain sent & \textbf{-4.73} & \textbf{-1.72} & 0.01 & -0.01 & \textbf{-4.79} & \textbf{9.50} & 0  & \textbf{-0.22} & \textbf{-1.40}  \\
Add definition ($\uparrow$) & -2.77 & -1.49 & 0.01 & 0.27 & -2.51 & -1.96 & -0.71 & -0.22 & -1.45\\
\midrule
\textbf{Simplification ($\uparrow$)} & -11.31  & -5.84  & -0.07  & -1.83 & -8.32  & \textbf{-15.45} & 0.10 & -0.55   & \textbf{1.02} \\
\midrule
\textbf{Coherence ($\downarrow$)} & \textbf{-1.28} & 0.01 & 0 & 0.05 & \textbf{-0.64} & \textbf{5.37} & \textbf{-1.75} & -0.03 & 1.0 \\
\midrule
% \multicolumn{8}{l}{\textbf{Faithfulness($\downarrow$)}}\\
\textbf{Faithfulness ($\downarrow$)} & & & & & & & \\
Number swaps & -0.70 & 0.49 & 0.01 & 0.46 & -0.39  & -2.96  & 3.04 & -0.09 & \textbf{-1.21} \\
Entity swaps & \textbf{-1.79} & -0.93 & \textbf{-0.01}  & 0.09  & \textbf{-1.33} & \textbf{8.96} & -0.01 & \textbf{-0.41} & 0.72  \\     
Synonyms verb swaps & -1.80 & -0.90 & -0.01  & 0.87 & -1.45  & 43.63  & 0  & -0.05 & 1.13 \\
Antonyms verb swaps & \textbf{-1.22} & -0.62  & -0.01  & 0.49 & \textbf{-1.31}  & \textbf{25.74}  & 0.03 & \textbf{-0.28} & 0.99 \\
Negate sentence & -0.86 & -0.30 & 0 & 0.33 & \textbf{-0.84} & \textbf{4.84} & 0 & \textbf{-0.67} & 0.22 \\
\midrule
\textbf{ACL'22 improvement} & 0.89 & 0.69 & 0.50 & 1.71 & 0.55 & -2.06 & - & - & - \\
\bottomrule
\end{tabular}

\caption{Slope coefficients of linear regression between perturbation percentage and automated evaluation metrics for CELLS. Slopes represent the estimated change in evaluation score for full perturbation. \textbf{Bold} indicates statistical significance in the correct direction with Bonferroni-Holm correction for multiple hypothesis testing \cite{holm1979simple}. We also provide the median reported score improvements from ACL'22 papers on text generation and summarization to help contextualize these deltas.}
\label{perturbation_slope}
\end{table*}


==> tables/plaba_dataset_description.tex <==
\begin{table}
\small
\centering
\begin{tabular}{@{}l l l@{}}
\toprule
 & \textbf{Src.} & \textbf{Tgt.} \\
\midrule
\textbf{Avg. \# words}  & 240 & 244\\
\textbf{Avg. \# sentences} & 10 & 12 \\
\bottomrule
\end{tabular}
\caption{PLABA dataset (n=750) statistics for source (abstract) and target (adaptations)}
\label{plaba_dataset}
\end{table}

==> tables/plainscore.tex <==
\begin{table*}[tbh!]
\centering
\small
\begin{tabular}{@{}cccccccccc@{}}
\toprule
\multicolumn{1}{l}{} & \multicolumn{3}{c}{\textbf{BioMedLM-PPL}}   & \multicolumn{3}{c}{\textbf{T5-PPL}}      & \multicolumn{3}{c}{\textbf{POMME}} \\
\cmidrule(lr){2-4}
\cmidrule(lr){5-7}
\cmidrule(lr){8-10}
\multicolumn{1}{l}{\textbf{Datasets}} & \textbf{Source}   & \textbf{Target}   & \textbf{$\Delta$ ($\uparrow$)} & \textbf{Source}   & \textbf{Target}   & \textbf{$\Delta$ ($\downarrow$)} & \textbf{Source}    & \textbf{Target}    & \textbf{$\Delta$ ($\uparrow$)}  \\
\midrule
CELLS                & -0.36 & 0.36  & \textbf{0.72}         & 0.52  & -0.52 & \textbf{-1.04}       & -0.88  & 0.88   & \textbf{1.76}         \\
\midrule
PLABA                & -0.79 & -0.14 & \textbf{0.65}         & 0.29  & 0.31  & 0.02        & -1.08  & -0.45  & \textbf{0.63}         \\
MSD                  & 3.30   & 3.30   & 0.0            & -1.89 & -1.94 & \textbf{-0.05}       & 5.19   & 5.24   & \textbf{0.05}         \\
WikiSimple           & 1.28  & 2.47  & \textbf{1.19}         & -1.12 & -3.23 & \textbf{-2.11}       & 2.40   & 5.70   & \textbf{3.30} \\
\bottomrule
\end{tabular}
\caption{BioMedLM-PPL, T5-PPL and \plainscore scores for four simplification datasets, comparing source (complex text) and target (simple text). A higher \plainscore score indicates a higher degree of text simplification. The difference, denoted $\Delta$, is calculated by subtracting the source score from the target score. \textbf{Bold} indicates statistical significance in the correct direction (i.e., target is simpler than source) with Bonferroni-Holm correction for multiple hypothesis testing \cite{holm1979simple}. The CELLS dataset functions as the reference in all \plainscore computations.}
\label{plain_score}
\end{table*}

% \begin{table}
% \small
% \centering

% \begin{tabular}{@{} l r r r r@{}}
% \toprule
% \textbf{Dataset}  & \textbf{Content}  & \textbf{Src.} & \textbf{Tgt.}  & \textbf{$\Delta$}\\
% \midrule
% CELLS      & Scientific texts & -1.40  & -0.21 & \textbf{1.19}\\
% MSD        & Medical references    & 0.96   & 1.01 & \textbf{0.05}\\
% WikiSimple & Wikipedia articles   & -0.81  & 0.81 & \textbf{1.62} \\
% % Newsela    & News articles & 0.88 & -1.02 \\
% \bottomrule
% \end{tabular}
% \caption{\plainscore values for existing simplification datasets, comparing source (complex version) and target (simple version). A higher \plainscore value indicated a higher degree of text plainness. The difference, denoted by $\Delta$, is calculated by subtracting the source score from the target score. Bold values indicate instances where the target score surpasses the source score.}
% \label{plain_score}
% \end{table}

==> tables/plainscore_perturbed_percentage.tex <==
\begin{table}[tb!]
\centering
\small
\begin{tabular}{@{}ccccc@{}}
\toprule
             & \multicolumn{2}{c}{\textbf{CELLS}} & \multicolumn{2}{c}{\textbf{PLABA}} \\
\cmidrule(lr){2-3}
\cmidrule(lr){4-5}           
\textbf{Perturb\%}  & \textbf{PPL}   & \textbf{\plainscore}   & \textbf{PPL}   & \textbf{\plainscore}   \\
\midrule
20\%         & \textbf{-44.81}    & -5.32       & 3.06      & -0.38       \\
40\%         & \textbf{-17.52}    & -0.88        & 5.01      & \textbf{0.69}        \\
60\%         & \textbf{-14.14}    & -0.29        & 4.59      & \textbf{0.83}         \\
80\%         & \textbf{-11.55}    & 0.27         & 3.38      & \textbf{0.76}        \\
100\%        & \textbf{-15.45}    & \textbf{0.42}        & 1.80      & \textbf{0.68}      \\
\bottomrule
\end{tabular}
\caption{Delta in PPL and \plainscore scores at various levels of perturbation. \textbf{Bold} indicates statistical significance in the correct direction with Bonferroni-Holm correction for multiple hypothesis testing \cite{holm1979simple}.}
\label{plain_score_perturbed_percentage}
\end{table}
